Unified Memcapacitor-Memristor Memory for Synaptic Weights and Neuron Temporal Dynamics

We present a fabricated and experimentally characterized memory stack that unifies memristive and memcapacitive behavior. Exploiting this dual functionality, we design a circuit enabling simultaneous control of spatial and temporal dynamics in recurrent spiking neural networks (RSNNs). Hardware-aware simulations highlight its promise for efficient neuromorphic processing.

==> Comments/comments_FM.tex <==
\begin{document}

\title{Comments from Filo}

\subsection{Section II: analog neuromorphic}
Not all neuromorphic is analog. So you might want to say:
"Analog In-Memory Neuromorphic computing is a promising approach for energy-efficient embedded sensory processing".

\subsection{Section II: FeCAP acronym is defined again}
It was already introduced in the Introduction, non need to define it again.

\subsection{Section II: what is the "wake-up effect"?}
Maybe include a reference if you don't have space to explane

\subsection{Section II: Rephrasing}
"We  characterized  FeCAPs  with  an  area  of 100μm2" sounds like it might either be the whole array or just a device. To disambiguate, rewrite as "We characterized FeCAPs with an per-device area of 100μm2".

\subsection{Section II: Figure 3 explanation}
Figure 3 is great! I am particularly impressed by how you smoothly integrated the programming pulses in the figure, looks very good! Just one thing, I understand that the programming pulse is what happens at the very begining, with the two strong polarizing pulses of opposive sign. Then, isn't the rest the read operation? Correct me if I am wrong. Otherwise, please specify what is READ and what is WRITE in the subplots.

Also, where is this voltage applied? 

\subsection{Figure 6: Change the names of the labels}
The labels are right now correct by they don't show that you are using FeCAP+RRAM data.
Heterogeneity: FeCAP + RRAM
Classic: CMOS + RRAM (right?)
Also, I would first plot the RSNN with 64 and then with 128 (just a viz preference).
\end{document}
